Benchmarking Distributional Alignment of Large Language Models

Language models (LMs) are increasingly used as simulacra for people, yet their ability to match the distribution of views of a specific demographic group and be \textit{distributionally aligned} remains uncertain. This notion of distributional alignment is complex, as there is significant variation in the types of attributes that are simulated. Prior works have underexplored the role of three critical variables -- the question domain, steering method, and distribution expression method -- which motivates our contribution of a benchmark explicitly addressing these dimensions. We construct a dataset expanding beyond political values, create human baselines for this task, and evaluate the extent to which an LM can align with a particular group's opinion distribution to inform design choices of such simulation systems. Our analysis reveals open problems regarding if, and how, LMs can be used to simulate humans, and that LLMs can more accurately describe the opinion distribution than simulate such distributions.

==> Sections/benchmark.tex <==
\label{sec:benchmark}
% The goal of this benchmark is to rank models and humans in their ability to be distributionally aligned to certain demographic groups given a particular steering method. We have two main leaderboards, one default setting that measure the distributional alginment task, and another that measures the knowledge to simulation gap. On top of this, we perform additional robustness checks and variations to see how model rankings hold.

In this section, we describe three main sources of variation in the distributional alignment task and how they are used to construct the benchmark. Then, we describe the human annotations collected to establish a human baseline for the distributional alignment task (Sec. \ref{sec:benchmark-human}).
% First, we vary the dataset and discuss its construction (Sec. \ref{sec:benchmark-datasets}).
% In the input, we vary the dataset and the steering method (Sec. \ref{sec:benchmark-steeringmethod}). In the output, we vary the distributional output type (Sec. \ref{sec:benchmark-estim-method}). 
% After these components are operationalized, we explain how the final leaderboards aggregate the sources of variation to reflect model performance  (Sec. \ref{sec:benchmark-leaderboard}).

\subsection{Source of Variation in the Distributional Alignment Task}
\subsubsection{Datasets}
\label{sec:benchmark-datasets}
% how the datasets are preprocessed 

In this section, we describe the desiderata of datasets for our benchmark, how OpinionQA \citep{santurkar2023opinions} is pre-processed for group opinion distributions, and the construction of a new non-political subjective opinion dataset, NYT Books.

\textbf{Dataset Desiderata: }An appropriate dataset to measure distributional alignment should include subjective questions with answers that vary across demographic groups, questions that we can easily extract opinion distributions from (e.g., multiple choice), and a reference human opinion distribution from each demographic groups from which we can compare LLMs. We can build this demographic group distribution by aggregating the human responses across answer choices and stratifying based on demographic group.\footnote{In practice, the set of demographic groups is limited by human annotations, as humans are steered towards each demographic group and then provide a group opinion distribution estimation.}

% we give a brief summary for the first 2, and discuss our new dataset in further detail.


\textbf{OpinionQA: }We use the OpinionQA dataset from \citet{santurkar2023opinions} to leverage public opinion surveys to compare the distribution of LLM responses to those of US citizens. In their steerability analysis, they create a smaller set of 500 contentious questions where the subgroups frequently disagree. We follow suit and randomly sample 100 question from this set to obtain questions spanning topics such as science, politics, and personal relationships from PEW Research’s American Trends Panel. We obtain the ground truth human opinion distributions of PEW survey respondents belonging to six demographic groups: Democrat, Republican, Male, Female, Black, and White.

% \subsubsection{Global Values \citep{durmus2024measuring} \nicole{TO DO}}


\textbf{NYT Books: } 
%Prior work in distributional alignment has primarily evaluated value-laden survey questions \citep{durmus2024measuring,santurkar2023opinions}, motivating our construction of a new dataset that provides better coverage over non-value-centric subjective tasks. 
There are now a number of works studying how LMs respond to political opinions or cultural values\citep{santurkar2023opinions,durmus2024measuring}, but it is less understood how LMs respond to non-political, yet still subjective values. 
How do our findings extend to other domains of personalization? Are LMs still suitable for this use case? 
% \irena{Interesting. The way you set this up makes me wonder if you could also use existing review datasets, e.g. IMDB, and then ask the model to simulate the distribution of human opinions about some movie. I guess you need a review dataset with demographic subsets.}

This motivates the construction of a new dataset, \textbf{NYT Books}, that gathers opinions on interest in the top books from the past two decades as judged by the NYTimes \citep{nytimes2024topbooks}. The purpose of NYT Books is to capture subjective values from demographic groups that are less directly measuring cultural values and political leanings, unlike the questions from OpinionQA which directly ask value-laden survey questions. 

\textbf{Annotation setup: } To construct this dataset, we gathered 235 books and their corresponding author, book summary, and genre. We asked 346 annotators to provide a 1-4 Likert rating to the following question, ``Given the summary of this book, how likely are you to read it?" for 26 books. From this data collection process, we surveyed 131 Male, 206 Female, 165 Democrat, and 172 Republican annotators, resulting in 18 annotations per book per demographic group. From these annotations, we calculated an opinion distribution over the 4 Likert ratings for each book. All crowd workers are sourced on Prolific, filtered for English fluency, selected from a pool of annotators who pass an attention check 93\% of the time, and are paid \$12 per hour. 

\NB{I feel like you can probably move some of these dataset construction details to appendix}

\NB{new paragraph header here? this paragraph looks long}
From analyzing the human annotations, we find NYT Books contains subjective questions with disagreement in book interest. On the left of Fig. \ref{fig:nytimes}, we plot the top 5 books that have the largest difference in Democrat and Republican annotator ratings.
Books that our Republican annotators preferred over Democrat annotators include works such as \textit{Redeployment} by Phil Klay (twelve stories by a former Marine who served in Iraq), \textit{Washington's Crossing} by David Hackett Fischer (a story from the American Revolutionary War) and \textit{Eastbound} by Maylis De Kerangal (a short novel about a young Russian soldier on a trans-Siberian train). Books that our Democrat annotators preferred over Republican annotators include works such as \textit{A Promised Land} by Barack Obama, \textit{A Short History Of Women} by Kate Walbert, \textit{Ten Thousand Saints} by Eleanor Henderson (a novel following a group of friends, lovers, parents and children through the straight-edge music scene and the early days of the AIDS epidemic), and \textit{Nw} by Zadie Smith (a modern novel illuminating questions of race, class, sexual identity and personal choice). \NB{I feel like this is way too much detail, maybe just a couple books that have high disagreement} 
Moreover, the Cohen's kappa of opinions with a demographic group is \nicole{X} and  Cohen's kappa of opinions between demographic groups is \nicole{X}.

% To demonstrate the distributional differences that we task LLMs to simulate, we plot the distribution of Likert ratings of two books, \textit{Washington's Crossing} by David Hackett Fischer and \textit{A Short History Of Women} by Kate Walbert, and observe a distinct distribution of Likert ratings (Fig. \ref{fig:nytimes}b),


\begin{figure}[ht!]
  \centering
  \includegraphics[width=\linewidth]{Figures/nytimes_final.pdf}
  \caption{Top 10 books that have the largest difference in Democrat and Republican annotator ratings, along with the 95\% confidence interval from bootstrapping with 1000 samples.}
\label{fig:nytimes}
\end{figure}






% 2 main leaderboards that vary in the amount of information they have



% 1. group information 
% 2. given distributional information 
% - for each we vary the model and the way distributions are expressed 
% - we want people to make progress on this!

% Variants/Analyses: 
% - increasing the number of question (n=100-->500)
% - increase amount of distributional information 
% - increasing the number of groups (n=6 --> n=14)

% \subsection{Default}
% This serves as our main leaderboard for ranking models and their steering method. We compare 9 models each with no steering, persona steering, and few shot steering. We rank these models on their ability to emulate a 6 distinct demographic groups (Democrat, Republican, Male, Female, Black, White) on the distributional alignment task.

% The default setting is evaluated on OpinionQA, Global Values, and NYTimes. 

% \subsection{Output Types}
% This setting is important as it reveals the models internal distributions are often misaligned with its verbalized distribution.2
% Variable we test: 
% \begin{itemize}
%     \item Sequence
%     \item Verbalize
%     \item Model Log Probs
% \end{itemize}
% Evaluated on opinionQA datasets


% \subsection{Training Data Regime}
% Understanding performance with and without access to training data: As we go from a low information to high information setting, how does model performance change? 
% Variable we test: 
% \begin{itemize}
%     \item No steering
%     \item Persona steering
%     \item Similar questions N=5 Easy Hard [Completed in [1]]
%     \item Similar questions N=5 Easy
%     \item Similar questions N=All other questions in the wave 
% \end{itemize}
% Evaluated on opinionQA datasets

\subsubsection{Steering Methods}

% \textbf{Steering Methods:}
\label{sec:benchmark-steeringmethod}

In this section, we supplement Sec. \ref{sec:problemsetting-input}  with additional details on implementation, demographic groups, and the ``No Steering" baseline.

\textbf{Persona Steering}: To implement persona steering, we instruct an LM to pretend to be a member of the target demographic group (e.g. ``Please simulate an answer from a group of Republicans."). For OpinionQA, we study steering 6 demographic groups, and for NYT Books we steer towards 4 demographic groups.

\textbf{Few Shot Steering}: To implement few shot steering, for each question, we calculate the top 10 most similar questions or books as identified from their text embeddings 
\citep{gao2022simcse}. We found that some of these questions may be near-duplicates, especially in opinion QA where a single PEW survey may include many variants of the same question. Thus, we filter for the hardest similar examples, namely the top 5 questions most distinct in output distribution. We provide those questions and their ground truth output distribution as few shot examples.
We do this to ensure that we provide topically coherent and similar examples, while avoiding cases where the model simply copies the distribution in the few shot examples. This tests the model's ability to generalize to new survey questions. 




\textbf{No Steering}: We can directly contrast these steered model to models that have not been steered, i.e., asking the question without any demographic or identity prompt. 
% \nicole{explain we have same demographic groups as persona; need to motivate why we avoid copying - topically coherent but distributional different in output which tests the model's ability to generalize, we want to - surveys contain similar questions }

%\nicole{I could describe easy, easyhard, all but one, but I want to move that analysis in the results to the appendix}


\subsubsection{Distributional Output Type}
\label{sec:benchmark-estim-method}

As discussed in Sec \ref{sec:problemsetting-output}, we study three ways of measuring a model's estimate of the group's opinion distribution: model log-probabilities, emitting a sequence, and verbalizing the distribution. For all settings, we provide the full prompts in the Appendix. 

\textbf{Model Log-probabilities: } A model's next token log probabilities assigned to each of the answer choices (e.g., ‘A’, ‘B’...) provide a sampling distribution by directly sampling from the model.

\textbf{30 Token Sequence: } We instruct the model to directly simulate 30 samples from a target group and emit a sequence of 30 answer choices. This distribution is limited by the number of tokens emitted in the sequence, as we are trying to estimate a continuous distribution from a finite number of tokens. 
Thus, we report a discretization error,
% the performance when the input probabilities to generate the sequence is equal to the ground truth group opinion distribution.
which corresponds to the error incurred when drawing 30 samples from the ground truth and computing the total variation based on these samples


% reveals complexity of simulating heterogenous human opinions 

\textbf{Verbalized Knowledge: } We instruct the model to express a target group's opinion distribution in its output text through a JSON format. (e.g., \texttt{\{A: 25\%, B: 20\%, C: 45\%, D: 10\%\}}).


% In this section we first describe the main task used to benchmark the difference in ability for various models coupled with different steering methods to be steered towards a distribution of opinions of a particular target demographic group may hold. Then we describe and motivate two other settings relevant to the main task. 



\subsection{Contextualizing Model Performance: Human Baseline Annotations}
    \label{sec:benchmark-human}


Given that the difficulty of the distributional alignment task is poorly understood, a comparison of human and LM performance on the same task helps contextualize if lower performance is due to the model or from the challenging nature of this task. Thus, we recruit crowd workers to complete the distributional alignment task, both with persona steering and few shot steering as the models are instructed to do. To our knowledge, we are the first to ask humans to complete this task of distributional alignment. \nicole{fact check}

\textbf{Annotation Setup. }
We use the same 100 questions from the OpinionQA dataset and 235 book summaries that we evaluated models on, thus allowing us to compare human performance against the suite LMs we evaluate. Each survey question or book summary receives four annotations of  estimated opinion distributions over answer choices. As with the models, the human annotators experience three steering methods: no steering, persona steering, and few-shot steering.

Using the Prolific platform, we crowdsource human annotations for the distributional alignment task. We restrict the demographics of annotators to match the groups that we study as it provided us an opportunity to do an in-group vs out-group analysis. We restrict our annotators to Democrat (73\%), Republican (27\%), Male (33\%), Female (67\%), White (84\%), and Black (16\%) for the OQA annotations. For the NYT annotations, our annotators are Democrat (69\%), Republican (31\%), Male (37\%), and Female (63\%). Each question from the OQA and NYT datasets is annotated four times. We compensate the workers at a rate of \$12 per 

\NB{again I feel like a lot of the gory details can go to the appendix -- ultimately people care about the basics of the dataset construction, the major design knobs, and then the results/takeaways. A lot of the stats and whatnot can either be summarized in figures/stated succinctly, or put in appendix}

\textbf{Quality control.}
To ensure annotation quality, we limit the task to workers with English fluency and ask survey participants to answer a reading attention check question which our annotators achieved 93\% on. 
%\nicole{as checked on the NYT annotations, could include time pr num_questions - appendix}

% It allows us to validate that our benchmark is measuring the correct metric and understand how difficult the distributional alignment task is for humans. \nicole{reword?}



%human baseline is not target to beat, rather to contextualize performance 

%best LMs are approaching performance of untrained snap judgements of humans, what this suggests is that LMs are not catastrophically bad and they can performance snap judgements, 
% LB suggests it might be possible to do better
% what our work does - helps us form a mental model of what lms are doing - they are snap judgements of humans - for low stakes tasks, this might be sufficient,but if there are higher stakes we need more than a snap judgement 
% placed LMs as at around humans - but humans are not what we;d want to use 
% would we ask humans to do this task? 
% 2 versions: LM retrieves the person, LM is a good simulator - pretend estimate is whats is going on 

% Finally, we also contextualize model performance by computing the performance when each answer option is equally likely to occur in the sequence, or the uniform distribution of answer choices.

% \begin{itemize}
%     \item Human annotations: How difficult is this task for humans to do? Do models outperform humans? can ingroup predict ingroup response? Can outgroup predict ingroup response?  
%     \item Consistency: our findings / rankings are consistent across datasets (3 of them) and output types?
% \end{itemize}
% We experiment with 3 different ways of expressing model distributions 
% Does the way  help with being susceptible to steering? 
% Ex: 
% Outputting the distribution as a sequence 

% All crowdworkers are sourced on Prolific, filtered for English fluency, and paid an average of \$XX per hour. 







==> Sections/benchmark_arxiv.tex <==
\label{sec:benchmark}

Having formalized the notation for distributional alignment, we explore how it can be improved by focusing on three understudied sources of variation: the distributional expression method ($\mathcal{O}$), steering method ($S$), and dataset ($Y$).
In this section, we explain how these elements are used to construct the benchmark and describe the human baseline.
\subsection{Distributional Estimation Method ($\mathcal{O}$)}
\label{sec:benchmark-estim-method}

% In this section, we formalize the steering method, output type, and evaluation metric.


\begin{figure*}[ht!]
  \centering
  \includegraphics[width=0.9\textwidth]{Figures/biasedcoinflip.pdf}
  \caption{\textbf{Biased Coin Flip}: We find that when the probability of heads is measured via model log-probabilities (left), the results are highly uncalibrated (this behavior is mitigated with temperature scaling (TS), shown in green). However, when the distribution is expressed through emitting a 30-token sequence of H or T (Sequence) or directly verbalizing the distributional knowledge (Verbalize Knowledge), we do not observe the same mis-calibration.}
\label{fig:biasedcoin}
\end{figure*}



% When LMs are asked to emulate a population's response to a multiple-choice survey question, there is no single ``correct" answer choice. Instead, the model output should match the \textit{distribution} of model opinions for each question across the set of multiple-choice answers

% A steered model's opinion distribution can be extracted three ways: model log-probabilities, prompting for a sequence of answer choices, and directly verbalizing distributional knowledge. 
In this section, we describe three distributional expression methods and demonstrate how distributional alignment is highly sensitive to the distribution estimation method.\footnote{Full prompts in \href{https://github.com/nicolemeister/benchmarking-distributional-alignment}{github.com/nicolemeister/benchmarking-distributional-alignment.}}


% When LMs are asked to emulate a population's response to a multiple-choice survey question, there is no single ``correct" answer choice. Instead, the model output should match the \textit{distribution} of model opinions for each question across the set of multiple-choice answers. 
% \NB{I feel like this point is v important and should be conveyed in the introduction, when you define distributional alignment}


% In our benchmark we are going to consider 3 ways of distribution estimation:  Present the 3 ways

% Previous work used log-probs, but there are issues. 
\textbf{1. Model Log-probabilities: }
A model's next token log probabilities assigned to each of the answer choices (e.g., ‘A’, ‘B’...) provide a sampling distribution by directly sampling from the model. This is the canonical distribution estimation method \citep{santurkar2023opinions, durmus2024measuring};
% A natural distribution estimation method is to measure the model's log-probabilities of the next token response for each answer choice \citep{santurkar2023opinions, durmus2024measuring}; 
however, prior work has found that these model log-probabilities have a concentrated probability mass on a few answer choices rather than more dispersed answers as seen in their corresponding human distributions \citep{durmus2024measuring}, especially in models trained with Reinforcement Learning from Human
Feedback (RLHF) \citep{christiano2023deepreinforcementlearninghuman}. 


\textbf{2. Sequence of Tokens: }While model log-probabilities represent drawing samples from a LM,
% \NB{are you saying here that you estimate log probs with sampling? this is new to the reader I think, so maybe should state this more clearly---this is also just because you're operating in the API setting right? that should be explained somewhere}, 
a model can also express its distributions by behaving as a sampler. We instruct a model to emit a sequence of 30 samples from the distribution (e.g., \texttt{ABBBAABDDBACBDB}). 
This method is advantageous when practitioners want to generate samples from an opinion distribution for simulation purposes.\footnote{This is inspired by a common synthetic data generation prompting technique that instructs LLMs to emit a sequence or batch of answers to generate diverse samples \citep{wang2023selfinstructaligninglanguagemodels,dubois2024alpacafarmsimulationframeworkmethods,si2024llmsgeneratenovelresearch}.} 
This distribution is limited by the number of tokens emitted in the sequence, as we are trying to estimate a continuous distribution from a finite number of tokens. 
Thus, we report a \textbf{discretization error}---the error incurred when drawing 30 samples from the ground truth distribution and computing the total variation based on those samples.

% exclusively use a language model for both sampling and distribution estimation (i.e., no external sampler). 
%This represents a model's ability to simulate its knowledge of a distribution.

\textbf{3. Verbalize Distributional Knowledge: } 
% \NB{I think you should try to stick to a specific terminology for each of these expression methods. A good way to stay consistent is to write out a table with all your notation and terms of art, and make sure you stick with it when writing the paper} 
Lastly, we can remove the requirement that models must sample from simulated humans and instruct a model to directly verbalize the distribution in the output text, without an estimation procedure or post-processing applied (e.g., text in a JSON format \texttt{\{A: 25\%, B: 20\%, C: 45\%, D: 10\%\}}).\footnote{While this verbalized knowledge can be fed into an external random sampler, it is not a sufficient output for downstream applications (e.g., piloting surveys) and existing approaches to simulating humans do not take this approach \cite{park2023generative,samuel2024personagymevaluatingpersonaagents}. Our later results suggest this approach may be fruitful as a distributional alignment method.}
% as practitioners often exclusively use a language model for both sampling and distribution estimation \citep{todo}.
This differs from the aforementioned methods in that it separates distributional knowledge from the LM's ability to also generate samples. 


% Simple experiment to show this log prob weakness. 
\textbf{These three estimation methods reveal surprising performance gaps.} Consider a toy experiment in which the model has \textit{full knowledge} of the ground truth distribution.
% Due to the __ of model log-probabilities, verbalize and sequence turn out to the extracted distribution is highly sensitive to the distribution estimation method.
% We demonstrate the magnitude of this issue with a toy experiment in which the model has \textit{full knowledge} of the ground truth distribution.
In this experiment, an LLM is instructed to simulate a flip of a biased coin which has $P(H)=p$ and $P(T)=1-p$. Naturally, we would expect the model log-probabilities for the token `H' to be $p$ and `T' to be $1-p$. In reality, we see that the model log-probabilities are highly un-calibrated. They provide a misleading picture of the ground truth distribution, despite the fact that the ground truth distribution is shared in the input prompt (Fig.~\ref{fig:biasedcoin}). Moreover, we find that two other distributional estimation methods do not suffer the same mis-calibration issue: both verbalizing the distribution and emitting a sequence of 30 samples of the biased coin flip are much more calibrated than the model's log-probabilities.\footnote{This performance gap is not unexpected; it has been shown that while models excel in text and image generation tasks (knowledge), they fall short when asked to validate if the generated answer is correct \citep{li2023benchmarking,west2023generative}.}
% \NB{the samples aren't IID though right? (otherwise they should do exactly as well as the log probs?) maybe should mention this, idk}




% This problem is fixed by using the other estimations → show sensitivity to distribution method  : Set up / motivate knowledge to simulation gap . We term this knowledge to simulation gap

% \nicole{todo: commentary on knowledge to sim}


Results from this biased coin flip experiment suggest two things: (1) prior distributional alignment work using model log-probabilities may not be seeing the full picture and (2) there exists a significant performance gap, one that we term \textit{knowledge-to-simulation gap}. This gap refers to instances where models may have alignment in knowledge (i.e., verbalizing the distribution in the output text), but not in sampling behavior (i.e., as measured via model log-probabilities or emitting a sequence of tokens). 

We define the \textbf{knowledge-to-simulation gap} as the percent error between the alignment when emitting a sequence of answer choices and verbalizing the distribution.\footnote{The gap can also defined as the difference in performance between verbalize and model log-probabilities, yet our later results show model log-probabilities to not be competitive.} More formally, this gap is: 
\begin{equation}
\label{eq:knowledge_to_sim}
    \text{KS}_S = \frac{\mathcal{A}(Y,\hat{Y}_{S, {\text{Sequence}}})}{\mathcal{A}(Y,\hat{Y}_{S, {\text{Verbalize}}})}-1.
\end{equation}


\subsection{Steering Method ($S$)}

% \textbf{Steering Methods:}
\label{sec:benchmark-steeringmethod}

Steerability in the context of this work refers to a LM’s ability to adapt to represent the opinion of a target demographic group.
We evaluate two steering methods, persona and few-shot steering, by prepending additional context to the prompt describing the group we want the model to emulate. 
We chose to study this few-shot setting, as it is known that persona steering can be inaccurate, leading to undesirable side effects including stereotyping, exacerbating polarization, and creating echo chambers \citep{perez2022discovering, cheng2023marked, wang2024large}.

% Persona Steering
\textbf{Persona Steering}: 
\citet{cheng2023marked} define a persona as a ``natural language portrayal of an imagined individual belonging to some (intersectional) demographic group.'' In persona steering, we append a persona to the prompt and ask the LM to emulate behavior from this group. Concretely, we follow a version of persona steering from \citet{santurkar2023opinions,Kambhatla} where the LM is instructed to pretend to be a member of the target demographic group (e.g. ``Please simulate an answer from a group of Democrats.''). 
%For OpinionQA, we study steering 6 demographic groups, and for NYT Books we steer towards 4 demographic groups.


% Few Shot
\textbf{Few Shot Steering}: 
% Despite its popularity, prior work has persona steering to be susceptible to stereotyping \citep{santurkar2023opinions,liu2024evaluating,wang2024large}.
Inspired by the success of few-shot prompting in language understanding tasks \citep{NEURIPS2020_1457c0d6}, 
we construct a few shot setting in which in-context examples of ground truth group opinion distributions are provided in addition to the persona. Specifically, LMs are given the top five most similar questions and their corresponding ground truth distribution from a group, and instructed to simulate an answer from that group (see Appendix~\ref{sec:appendix-fewshot} for more details). This setting is representative of when practitioners have access to existing survey data for similar questions. 


%To implement few shot steering, 




\textbf{No Steering}: We can directly contrast steered models to models that are prompted with a question without any demographic or identity markers. 
% \nicole{explain we have same demographic groups as persona; need to motivate why we avoid copying - topically coherent but distributional different in output which tests the model's ability to generalize, we want to - surveys contain similar questions }

%\nicole{I could describe easy, easyhard, all but one, but I want to move that analysis in the results to the appendix}


%Goal: there are a couple different steering methods, steering methods are important. 


\subsection{Dataset ($Y$)}
\label{sec:benchmark-datasets}
% how the datasets are preprocessed 

In this section, we describe three datasets for quantifying distributional alignment -- OpinionQA~\citep{santurkar2023opinions}, GlobalOpinionQA~\citep{durmus2024measuring}, and a new non-political subjective opinion dataset, NYT Book Opinions.

% \textbf{Dataset Desiderata: }An appropriate dataset to measure distributional alignment should include subjective questions with answers that vary across demographic groups, questions that we can easily extract opinion distributions from (e.g., multiple choice), and a reference human opinion distribution from each demographic groups from which we can compare LLMs. We can build this demographic group distribution by aggregating the human responses across answer choices and stratifying based on demographic group.\footnote{In practice, the set of demographic groups is limited by human annotations, as humans are steered towards each demographic group and then provide a group opinion distribution estimation.}

% we give a brief summary for the first 2, and discuss our new dataset in further detail.


\textbf{OpinionQA: }We use the OpinionQA dataset from \citet{santurkar2023opinions} to leverage public opinion surveys to compare the distribution of LLM responses to those of US citizens. In their steerability analysis, they create a smaller set of 500 contentious questions where the subgroups frequently disagree. We follow suit and randomly sample 100 questions from this set to obtain questions spanning topics such as science, politics, and personal relationships. We obtain the ground truth human opinion distributions of PEW survey respondents belonging to six demographic groups: Democrat, Republican, Male, Female, Black, and White.


\textbf{GlobalOpinionQA:}
GlobalOpinionQA consists of questions and answers from two cross-national surveys, World Values Survey and PEW Global Attitudes Survey. It is aimed at capturing diverse perspectives on global issues across various countries and is inspired by ~\citet{santurkar2023opinions}. We filter this dataset for the top 100 questions with the highest disagreement between pairs of countries as measured by the distance between the text embedding \citep{gao2021simcse} of the questions. See Sec.~\ref{sec:appendix-GV} for more details. 



\textbf{NYT Book Opinions: } 
%Prior work in distributional alignment has primarily evaluated value-laden survey questions \citep{durmus2024measuring,santurkar2023opinions}, motivating our construction of a new dataset that provides better coverage over non-value-centric subjective tasks. 
Several works study how LMs respond to political opinions or cultural values \citep{santurkar2023opinions,durmus2024measuring}, but it is less understood how LMs respond to non-political, yet still subjective values. 
How do our findings extend to other domains of personalization? Are LMs still suitable in this use case? 

This motivates the construction of a new dataset, \textbf{NYT Book Opinions}, that gathers opinions on interest in the top books from the past two decades as judged by \citet{nytimes2024topbooks}. The purpose is to capture subjective values that less directly measure cultural values and political leanings.
%, unlike the questions from OpinionQA which directly ask value-laden survey questions. 

\textbf{Annotation setup: } We collected 235 books and their corresponding author, book summary, and genre. 346 annotators provided a 4-point Likert rating to the question, ``Given the summary of this book, how likely are you to read it?'' for 26 books. See Sec.~\ref{sec:NYT-construction} for additional details.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{Figures/nytimes_final.pdf}
  \caption{Top 4 books with the largest difference between Republican and Democrat ratings (left) and the top 4 books with the largest difference between Democrat and Republican ratings (right), with a 95\% confidence interval from bootstrapping. }
\label{fig:nytimes}
\end{figure}





From these human annotations, we find disagreement in book interest. In Fig.~\ref{fig:nytimes}, we plot the top 4 books that have the largest difference in Democrat and Republican annotator ratings.
Books that Republican annotators preferred over Democrat annotators include works such as \textit{Redeployment} by Phil Klay (twelve stories by a former Marine who served in Iraq) and \textit{Washington's Crossing} by David Hackett Fischer (a story from the American Revolutionary War). Books that Democrat annotators preferred over Republican annotators include works such as \textit{A Promised Land} by Barack Obama and 
\textit{A Short History Of Women} by Kate Walbert.

% \NB{I feel like this is way too much detail, maybe just a couple books that have high disagreement} 
% Moreover, the Cohen's kappa of opinions \textit{within} a demographic group is \nicole{X} and  Cohen's kappa of opinions \textit{between} demographic groups is \nicole{X}.

% To demonstrate the distributional differences that we task LLMs to simulate, we plot the distribution of Likert ratings of two books, \textit{Washington's Crossing} by David Hackett Fischer and \textit{A Short History Of Women} by Kate Walbert, and observe a distinct distribution of Likert ratings (Fig. \ref{fig:nytimes}b),





% 2 main leaderboards that vary in the amount of information they have



% 1. group information 
% 2. given distributional information 
% - for each we vary the model and the way distributions are expressed 
% - we want people to make progress on this!

% Variants/Analyses: 
% - increasing the number of question (n=100-->500)
% - increase amount of distributional information 
% - increasing the number of groups (n=6 --> n=14)

% \subsection{Default}
% This serves as our main leaderboard for ranking models and their steering method. We compare 9 models each with no steering, persona steering, and few shot steering. We rank these models on their ability to emulate a 6 distinct demographic groups (Democrat, Republican, Male, Female, Black, White) on the distributional alignment task.

% The default setting is evaluated on OpinionQA, Global Values, and NYTimes. 

% \subsection{Output Types}
% This setting is important as it reveals the models internal distributions are often misaligned with its verbalized distribution.2
% Variable we test: 
% \begin{itemize}
%     \item Sequence
%     \item Verbalize
%     \item Model Log Probs
% \end{itemize}
% Evaluated on opinionQA datasets


% \subsection{Training Data Regime}
% Understanding performance with and without access to training data: As we go from a low information to high information setting, how does model performance change? 
% Variable we test: 
% \begin{itemize}
%     \item No steering
%     \item Persona steering
%     \item Similar questions N=5 Easy Hard [Completed in [1]]
%     \item Similar questions N=5 Easy
%     \item Similar questions N=All other questions in the wave 
% \end{itemize}
% Evaluated on opinionQA datasets




\subsection{Human Baseline Annotations}
\label{sec:benchmark-human}
Inspired by~\citet{yudkin_hawkins_dixon_2019} who study the \textit{Perception Gap}, or the percentage difference between a respondent’s estimate of how many people hold a certain view and the actual percentage of people who hold that view, we recruit crowd workers to complete the distributional alignment task. Annotators receive the same questions from OpinionQA and NYT Book Opinions that we evaluated models on, allowing us to compare human performance against the suite of LMs we evaluate. Due to challenges in accurately capturing culturally specific perspectives, we do not collect human annotations on GlobalOpinionQA. Estimating the opinions of respondents from different countries would require annotators with deep, contextually relevant knowledge of each country’s sociocultural landscape and it is well established that annotations from Western populations do not accurately reflect non-western views~\citep{APICELLA2020319,Arnett2008TheN9}. This decision was made to ensure that conclusions drawn are not confounded by culturally mismatched interpretations.
As with the models, the human annotators are shown three prompts including no steering, persona steering, and few-shot steering. Each survey question receives four annotations, or human estimates of opinion distributions over answer choices.

%\nicole{as checked on the NYT annotations, could include time pr num_questions - appendix}

% It allows us to validate that our benchmark is measuring the correct metric and understand how difficult the distributional alignment task is for humans. \nicole{reword?}



%human baseline is not target to beat, rather to contextualize performance 

%best LMs are approaching performance of untrained snap judgements of humans, what this suggests is that LMs are not catastrophically bad and they can performance snap judgements, 
% LB suggests it might be possible to do better
% what our work does - helps us form a mental model of what lms are doing - they are snap judgements of humans - for low stakes tasks, this might be sufficient,but if there are higher stakes we need more than a snap judgement 
% placed LMs as at around humans - but humans are not what we;d want to use 
% would we ask humans to do this task? 
% 2 versions: LM retrieves the person, LM is a good simulator - pretend estimate is whats is going on 

% Finally, we also contextualize model performance by computing the performance when each answer option is equally likely to occur in the sequence, or the uniform distribution of answer choices.

% \begin{itemize}
%     \item Human annotations: How difficult is this task for humans to do? Do models outperform humans? can ingroup predict ingroup response? Can outgroup predict ingroup response?  
%     \item Consistency: our findings / rankings are consistent across datasets (3 of them) and output types?
% \end{itemize}
% We experiment with 3 different ways of expressing model distributions 
% Does the way  help with being susceptible to steering? 
% Ex: 
% Outputting the distribution as a sequence 

% All crowdworkers are sourced on Prolific, filtered for English fluency, and paid an average of \$XX per hour. 








==> Sections/experiments_arxiv.tex <==
\label{sec:experiments}

We rank GPT-4, GPT-3.5, Anthropic Haiku, Anthropic Opus, Llama-3 70B Instruct,\footnote{Smaller models struggled to follow the sequence distribution expression method, thus restricting our model selection.} based on distributional alignment (Eq.~\ref{eq:distributional_alignment}) and the knowledge-to-simulation gap (Eq.~\ref{eq:knowledge_to_sim}), and average across groups, steering methods, and datasets. 
We start by describing the performance on the distributional alignment task.
Then, we dive into the implications that emerge from varying the distribution expression method, dataset, and steering method. 
\NB{I feel like you start experiments with the key questions you want to answer and also maybe some headline results that you find. if you end up going with the more active pitch of "verbalized distributions perform best" you could mention this here, I think}

% \subsection{Setup}
% \label{sec:exp-setup}


% We 
% \textbf{Distributional Alignment Task:} In the main task, we evaluate models based on the average total variation between the model output distribution and ground truth group distribution,
% $\mathcal{A_{\texttt{Verbalize}}}$, where a lower distance represents higher distributional alignment. We average over groups, steering methods, and datasets and report results from the ``verbalize" distributional output type. 

% \textbf{Knowledge-to-Simulation Gap:} We evaluated models based on the knowledge-to-simulation-gap, as defined in Sec. \ref{sec:problemsetting-output} and \ref{sec:problemsetting-eval}. We average across groups, steering methods, and datasets. 


% \nicole{meta-discursive voice}
\subsection{Distributional Alignment Performance}
\label{sec:exp-performance}

% TABLE WITH: OQA AND NYT AND GV
\begin{table}[ht!]
  \centering
  \begin{minipage}{\linewidth}
    \centering
    \begin{tabular}{ll}
      \toprule
      Model     & $\mathcal{A}(Y,\hat{Y}_{\mathcal{S}, \mathcal{O}})$  \\
      \midrule
\rowcolor{lightgray} Anthropic Opus (V)  & 0.226 $\pm$ 0.006 \\ 
\rowcolor{lightgray} GPT-4 (V)           & 0.229 $\pm$ 0.006 \\ 
\rowcolor{lightgray} Llama 3 70B (V)     & 0.244 $\pm$ 0.006 \\ 
\rowcolor{lightgray} Anthropic Haiku (V) & 0.254 $\pm$ 0.007 \\ 
GPT-4 (TS-Log-p)      & 0.273 $\pm$ 0.006 \\ 
GPT-4 (Seq)           & 0.278 $\pm$ 0.008 \\ 
\rowcolor{lightgray} GPT-3.5-Turbo (V) & 0.291 $\pm$ 0.007 \\ 
GPT-3.5-Turbo (TS-Log-p) & 0.296 $\pm$ 0.006 \\ 
Anthropic Haiku (Seq) & 0.309 $\pm$ 0.006 \\ 
GPT-3.5-Turbo (Seq)  & 0.318 $\pm$ 0.007 \\ 
Anthropic Opus (Seq)  & 0.325 $\pm$ 0.007 \\ 
Llama 3 70B (Seq)     & 0.328 $\pm$ 0.008 \\ 
GPT-3.5-Turbo (Log-p) & 0.455 $\pm$ 0.008 \\ 
Llama 3 70B (TS-Log-p) & 0.469 $\pm$ 0.009 \\ 
Llama 3 70B (Log-p)    & 0.495 $\pm$ 0.008 \\ 
GPT-4 (Log-p)         & 0.550 $\pm$ 0.008 \\ 
            \midrule
            Discretization Error (Seq) & 0.115 $\pm$ 0.004  \\
            Uniform & 0.363 $\pm$ 0.007   \\
            Majority Vote & 0.712 $\pm$ 0.013 \\ 
            % Minority Vote & 0.846 $\pm$ 0.011 \\ 
      \bottomrule
    \end{tabular}
    \subcaption{\textbf{Distributional Alignment Task}. Models ranked based on mean total variation distance. Models highlighted in gray and with (V) have a distribution expression method of directly verbalizing the distribution in a JSON format ($\mathcal{O} = \texttt{Verbalize}$). Models not highlighted represent samplers, where (Seq) represents the 30-token sequential distribution output ($\mathcal{O} = \texttt{Sequence}$), (Log-p) represents $\mathcal{O} = \texttt{Model Log-probabilities}$, and (TS-Log-p) represents $\mathcal{O} = \texttt{Temperature Scaled Model Log-probabilities}$. }
    \label{tab:main-a}  
    
% \hspace{0.1\textwidth} % Adjust spacing between tables if needed

  \end{minipage}%
  \hspace{0.01\textwidth} % Adjust spacing between tables if needed
  \begin{minipage}{\linewidth}
    \centering
    
    \begin{tabular}{lc}
      \toprule
      Model     & Simulation Penalty     \\
      \midrule
GPT-3.5 Turbo & 9.17\% \\ 
GPT-4 & 21.35\% \\ 
Anthropic: Haiku & 21.49\% \\ 
Llama 3 70B Instruct & 34.65\% \\ 
Anthropic: Opus & 43.63\% \\ 
      \bottomrule
    \end{tabular}
    
    \subcaption{\textbf{Knowledge-to-Simulation Gap (Eq.~\ref{eq:knowledge_to_sim})}. The simulation penalty measures the percent error increase in total variation between the 30-token sequential distribution output and the verbalization of knowledge.}
    \label{tab:main-b}
  \end{minipage}
\caption{\textbf{Model Performance}. In both tables, we and rank models from highest to lowest performance on the task and average over all three datasets, persona and few shot steering, and all demographic groups. We report the 95\% confidence interval from bootstrapping with 1000 samples.}
\end{table}






In Tab.~\ref{tab:main-a}, we report the results of our distributional alignment leaderboard where we rank models on their ability to be steered towards a demographic group, averaged over persona steering and few shot steering, and all three datasets. In this leaderboard, where lower numbers represent higher distributional alignment, we find that verbalizing the distribution results in higher performance, with Anthropic Opus and GPT-4 being the most steerable amongst our models. These numbers can be directly compared to the performance of the uniform baseline, where each answer option is equally likely to occur in the sequence (0.363), a majority vote baseline, where the ground truth distribution is compared to a distribution in which all the probability mass is placed on the highest likelihood ground truth answer choice (0.707). 
% , and minority vote baseline, where the ground truth distribution is compared to a distribution in which all the probability mass is placed on the least likelihood ground truth answer choice (0.846).
% We also evaluate human performance on the distributional alignment task, and find that all models except GPT-3.5 outperform humans. 

\subsection{Implications for Distributional Alignment}
\label{sec:exp-implications}
In this section, we organize our analyses into implications for the field and conclude each section with actionable suggestions for practitioners who use LLMs for simulating human subjects.
% \NB{ I feel like this is the nice active framing that you should try to have throughout}

%  Finally, we dive into the find-488
% ings and implications that emerge from varying489
% the distribution output type, dataset, and steering490
% method

% \NB{I would define the knowledge to simulation metric here, directly after noting from the experiments that verbalized strictly dominates sampling}
\textbf{A large knowledge-to-simulation gap exists. }As observed in Sec.~\ref{sec:benchmark-estim-method}, even when a model knows as distribution, sometimes it cannot sample it. To this end, we measure these gaps between knowledge and simulation in our second leaderboard (Tab.~\ref{tab:main-b}). We observe that some models, particularly those from the Llama-3 and Anthropic suite have a larger knowledge-to-simulation gap, especially when directly compared to the OpenAI models. This highlights room for improvement, as the language model is capable of returning more accurate estimates of human opinions when expressing the distribution through verbalizing the distribution, but not when simulating samples from this distribution.
\textbf{\textit{Implication: }}If practitioners are using models with a high knowledge-to-simulation gap, they should prompt the model to verbalize the knowledge directly and use an alternative sampler for simulation purposes.
\NB{shouldn't the implication be: if you want the distribution, use verbalized; if you want samples, still used verbalized, but use an external sampler?}
% When decoupling the knowledge of a distribution and the ability to simulate the distribution, we find a significant knowledge-to-simulation gap, in which LLMs can return accurate estimates of human opinions, but struggle to simulate samples from this distribution. 

% \begin{figure*}[ht]
%   \centering
%   \includegraphics[width=\textwidth]{Figures/logprobs_bad.pdf}
%   \caption{Model Log-probabilities gives us a misleading picture of distributional alignment. We average the performance of the distributional alignment task over all datasets and steering methods.\nicole{will add llama3-70b log probs} 
%   % \NB{wait, what is the super good seq one? reading this figure it looks like that one is just "discretization error" lol}
%   }
%   \label{fig:badlogprobs}
% \end{figure*}

\textbf{Model log-probabilities can be misleading.} Next, we highlight a larger knowledge-to-simulation gap between model log-probabilities and the verbalization of knowledge (Tab.~\ref{tab:main-a}). Using model log-probabilities to measure distributional alignment results in worse performance than even \textit{uniform} distribution on the distributional alignment task. We find that this performance gap can be in part attributed to log probabilities having a highly concentrated probability mass on one or two answer choices, as observed in \citet{durmus2024measuring} and our biased coin flip experiment from Sec.~\ref{sec:benchmark-estim-method}.
While prior work \citep{santurkar2023opinions,durmus2024measuring} has used model log-probabilities for steering and alignment applications, this distribution expression method \textit{underestimates} LLM capabilities in emulating demographic groups. Furthermore, we find that temperature-scaled model log-probabilities improve GPT-3.5 and GPT-4 results, but not for Llama-3-70B (Sec.~\ref{sec:appendix:TS}).
\textbf{\textit{Implication: }} We encourage practitioners to use alternative distribution estimation methods, such as emitting a sequence or verbalizing the distributional knowledge.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{Figures/oqa_vs_nyt.pdf}
  \caption{\textbf{Steering Method and Dataset: } We plot the average total variation for each dataset and steering method, averaged across demographic groups for the 30-token sequential distribution output. We find it is harder to steer models toward the dataset where opinions are hidden under a layer of abstraction (NYT). Additionally, few shot steering improves distributional alignment for humans and all models except for GPT-3.5.  \NB{could you maybe make some other strong claims based on these results? in particular it looks like GPT-4 is competitive or better than the human baseline -- that's pretty interesting/notable/a kinda flashy headline result?}}
  \label{fig:OQAvsNYT}
\end{figure}


    
\textbf{Steering is more challenging in non-cultural and non-political settings. }
The goal of the NYT Book Opinions dataset is to capture subjective values from demographic groups that less directly measure cultural values and political leanings, unlike OpinionQA questions which directly ask value-laden survey questions. We find that all models and humans are more easily steered towards questions in the OpinionQA dataset than the NYT Book Opinions dataset, as the total variation decreases from no steering to persona and few shot steering.
In Fig.~\ref{fig:OQAvsNYT}, we plot the average total variation for each dataset and steering method, averaged across demographic groups, for the output type of sequence. 
This suggests that when the values are hidden under a layer of abstraction (i.e., book interest) it may be harder to steer models towards the opinions of demographic groups. 
\textbf{\textit{Implication:} }When practitioners use LLMs to pilot survey questions that less directly allude to cultural values, they need to consider the nature of their questions and if LLMs are suitable for their use case. 
% \nicole{will include same analysis for model log prob and verbalize}

\textbf{Few shot steering improves persona steering. }   
For humans and all models except GPT-3.5, we observe statistically significant improvements in few shot steering over persona steering (Fig.~\ref{fig:OQAvsNYT}). As expected, when models have access to five examples of distributional data, they improve their distributional estimation capabilities.
\textbf{\textit{Implication: }}Practitioners should use prior distributional data as few shot examples over just personas, if possible.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{Figures/Dem_Repub_Stereotyping.pdf}
  \caption{\textbf{Models assume Democrats read more than Republicans.} In this plot, we show the marginal distribution of Likert Rating (1-4) in responses to the following question: ``How likely are you to read this book?'' A Likert rating of 1 refers to ``Very unlikely'' and a Likert rating of 4 refers to ``Very likely''. 
  We averaged over 235 questions from NYT Book Opinions and 5 models steered towards Democrats and Republicans with persona steering (orange) and few shot steering (green). In blue, we plot the reference human reference for Democrat and Republican annotators. We find that persona steering produces more stereotypical results.}
  \label{fig:NYT_stereotyping}
\end{figure}



\textbf{Persona-steered LLMs are susceptible to stereotyping. }Consistent with prior work studying persona steering and LLMs emulating human behavior \citep{gupta2024biasrunsdeepimplicit,cheng2023marked,cheng2023compostcharacterizingevaluatingcaricature,wan2023personalizedstochasticparrotsdangerous}, we find that the LLMs produce stereotypical outputs. For example, when analyzing the marginal distribution of the answer ratings in the NYT Book Opinions dataset (Fig.~\ref{fig:NYT_stereotyping}), we find that models prompted with a Democrat persona tend to simulate humans that are more likely to read books---the average simulated human has a 13\% chance of responding with ``very unlikely to read'' when our human annotators had a 33\% chance. Furthermore, the simulated Democrat has a 25\% chance of responding with ``very likely to read'', when our human annotators had a 12\% chance. This gap is significantly reduced when using few-shot steering. \textbf{\textit{Implication: }}It is important to collect disaggregated evaluation metrics to understand potential discrepancies between groups \citep{barocas2021designingdisaggregatedevaluationsai}. These findings support using prior distributional data as a few shot examples. 


% \textbf{Benchmark Ablations. } We perform additional robustness checks and variations to see how model rankings hold. \nicole{might table this for appendix..}
% \begin{enumerate}
%     \item Coverage: We extend beyond steering towards 6 groups to steer towards 14 total demographic groups for the OpinionQA dataset. This to better understand how models representing the opinions of minority groups compared to majority groups. We find that \nicole{todo} 
%     \item Number of survey questions in evaluation: We increase the number of survey questions evaluated on from 100 to 500 for the OpinionQA dataset and find \nicole{todo} ...



==> Sections/intro_old.tex <==
\label{sec:intro}

% Openining distributional values 
% people want to simulate people 

% Goal of P1: 
    % this is the problem setting
    % this is the problem
    % here is what is lacking
    
It would be unusual to ask a person to accurately simulate a demographic group to which they do not belong. However, LMs are increasingly being used to simulate human behavior, in applications ranging from agent-based simulations \citep{park2023generative} to studying human behavior from internet data \citep{buttrick2024} to piloting survey design \citep{hwang2023aligning, zhou2024sotopia, pmlr-v202-aher23a, ziems2024large,Argyle_2023}. 
% \irena{I would move the last sentence here and explicitly say, it's important to evaluate if these simulations are aligned with the intended human distribution.}
It is important to evaluate if these simulations are aligned with the intended human distribution as some have argued that the extensive training corpus of LLMs enables them to faithfully simulate demographic groups \citep{grossman2023}, while others have shown evidence that such simulations are inaccurate and stereotypical \citep{liu2024evaluating,wang2024large}. 
% P2: Describe what is lacking in current works surrounding distributional alignment, motivate development of a benchmark
% Introduce our new benchmark with new data
% MOTIVATE BENCHMARK & describe what is lacking in current works surrounding distributional alignment 

%(where an LM is given either no instruction or a simple persona)
% \irena{Nit, but I'm left askingif the results you cite in the first paragraph (Myra's paper, etc.) use the same methodology as Esin's work, or are they different?}
Distributional alignment is motivated by the fact that there is no single ``correct" answer choice to an opinion survey. Thus, the model output should match the \textit{distribution} of model opinions for each question across the set of multiple-choice answers. 
Current approaches to measuring these capabilities have focused on zero-shot, log-probability based evaluations 
% \irena{I would be more specific: not just zero-shot instead of few-shot, but multiple choice instead of generative}
of political or cultural values (e.g., the PEW and World Values Surveys \citep{santurkar2023opinions,durmus2024measuring}). 
\nicole{justify why these 3 varaibles are important, there is disagreement on if this should be done; is alignment robust across different settings? here is contradicting literature - therefore we study why they are different; dataset and distribution expression method is most important - highlight papers that talk about personalizaiton/robustness across topics/formats - we begin to answer some of these motivation questions p1: format p2: books. }
While these are important steps, the space of distributional, pluralistic alignment, where the goal is to accurately simulate the distribution of human preferences and opinions \citep{sorensen2024roadmap}, is much larger and is highly dependent on the setting. 
% \irena{I wonder if you can break down this term "distributional pluralistic alignment" a little more: what concretely does this mean? Or if your point is that this doesn't have a crisp meaning, expand more on how Taylor defines it. Feels like you're assuming familiarity with his work/ leaning on it to provide the definitions.}. 
In practice, there is significant variation in the types of attributes that are simulated (e.g., political opinions or product preferences), how the model expresses the distribution (having the model generate samples from the distribution or directly returning the distribution as text), and the steering method (adapting to represent the opinion of a target demographic group with few-shot examples or a text-based group description).

% \irena{Hmm, I got a bit lost. This is a bigger comment, building off of the previous one: can you make a note on what the inputs / outputs are when one runs a simulation? Are you asking interview questions? Evaluating monologues generated by personas? Asking for a description of the distribution? Later on, I think I understand that your point is that you're trying all of these: the way you probe the model's understanding of the distribution (generative vs. multiple choice vs. descriptive) affects its measured faithfulness. In that case, I would present the intro like this: ``People use LMs for simulation. It's improtant to ask if they are aligned with the human distribution, and honestly the definition of ``aligned'' is not very clear in prior work. To check ``alignment'', you can imagine probing the LM using X and Y and Z methods (each with their own evaluation metric), of which most works have tried only one. We show that X, Y, Z elicit very different behaviors from the LM, and the LM can appear aligned under one mode and not the other.''}

% \NB{the last point feels less about how you extract the responses and more about how the model expresses the distribution? also that seems like a higher-order concern than zero-shot versus few-shot, I might consider entirely omitting that part or perhaps only mentioning it in related work }
% \irena{+1 to Neil's comment, I also feel like there's some conflation of lower-level things (e.g., the specific prompt, or one-shot vs. few-shot) compared to this high-level question of how you interact with the LM to evaluate alignment.}

% In this work, we operate in the setting 

% Define steering, estimation method, 




\begin{figure*}[ht!]
  \centering
  \includegraphics[width=\textwidth]{Figures/Distributional Alignment Fig 1 (Final) (1).pdf}
  \caption{
  % \NB{also lol this is a very spicy figure 1... maybe too spicy? not sure}
  Our work studies how variations in the dataset (yellow), steering method (green), and distributional output type (purple)
  % \NB{I feel like you need a more active terminology than "output type". maybe method of expression? distributional expression method?}
  affect the quality of distributional alignment. We rank models and humans in their ability to align with the opinion distribution of demographic groups and find existing metrics for distributional alignment (i.e., model log-probabilities) systematically underestimate LM performance. While LMs may `know' about distributional alignment, they struggle to sample from their own distribution. 
  % \NB{final sentence doesn't match the penultimate, it should be optimistic about how you find some better way of expressing the opinion distribution right? one simple trick to get good opinion distribution expressions from LLMs?}
  }
%\href{https://docs.google.com/drawings/d/1_41Gn5htIfQm8m1dQxMpjYAo7nNCEA95kRqbXkaEfQ0/edit?usp=sharing}{google drawing link}
\label{fig:fig1}
\end{figure*}



In this work, we focus on alignment in multiple-choice opinion surveys, and build a benchmark to study such variation (Fig. \ref{fig:fig1}). We perform analyses that show how the performance of LLMs in distributional alignment tasks can be highly sensitive to (1) design choices in the dataset, (2) the steering method, and (3) the distribution expression method. We contextualize our results and analyses through new human baseline measurements that demonstrate these tasks are underspecified and very difficult.

Our analyses reveal several open problems for the field. First, existing benchmarks that measure the model's distribution with log-probabilities may have systematically underestimated LLM capabilities in emulating demographic groups. When expressing the distribution as in a text-based (e.g., `return the distribution in a JSON') or sequential (e.g., `sample 30 answer choices from this group') format, there are significant improvements for all tested models.
Next, these expressions of distributions in a text-based format (where language models do not generate samples but instead respond with the distribution written out) much more closely match the ground-truth than the sampling distribution. 
This highlights substantial opportunity for improvement in distributional alignment as a language model can sometimes return accurate estimates of human opinions, but the same model is often incapable of simulating samples from this distribution.
This gap is problematic as the verbalized distributions are less useful in downstream applications and generative settings, yet have highest performance.  \nicole{shorten}
% \NB{Not sure how this paragraph is different from the previous---are you basically saying that the verbalized distributions can much more closely match the ground-truth than the sampling distribution?}

% \nicole{insert a paragraph on how this paper reveals open problems}

Finally, we show the importance of additional human annotations, both in the types of questions we ask and in collecting human baselines for the distributional alignment task. When subjective survey questions indirectly capture cultural values or political leanings (e.g., book ratings, movie ratings), we find it is harder to steer models towards the opinions of demographic groups. 
\NB{is there a clearer way to say this? sounds to me like: when the questions reflect cultural/political values, distributional alignment is harder (maybe it would help to draw a comparison to what sorts of questions are easy?}
Additionally, we collect human annotations for this task and find that distributional alignment is challenging even for humans, which raises the question of how far distributional alignment can be improved in LMs that are trained primarily to imitate humans. 
\NB{the latter claim seems a little speculative, it seems plausible to me that being trained on the mixture of opinions on the internet can result in an LLM that is well-distributionally-aligned, even if there are no instances on the internet of people directly expressing opinion distributions}
% \irena{One piece that seems to be missing: during evaluation, we can probe the model in X,Y,Z ways, which is great. But when people are actually using models for simulations, what are they interested in? E.g., asking the model to describe the distribution in a JSON doesn't seem that useful to people trying to build artificial students to train teachers. I think you're hinting at this in the last couple of paragraphs, but I would state it explicitly: e.g., the generation stuff is what people actually want, but we find that this is where LMs are the weakest.}

% P6: Motivate benchmark + new dataset 
% Our distributional alignment benchmark 
% that allows us to better understand how models can be steered.
% In this paper, we first describe the broader goal of distributional alignment, then detail the construction of our new benchmark on distributional alignment tasks. Finally we discuss the results of evaluating models and steering methods using this benchmark. 


% P6: Our key contributions 

Our contribution is a \emph{distributional alignment benchmark} that exposes many key design choices and expands existing benchmarks through new domains and human baselines that are crucial for understanding LM alignment capabilities more holistically. We summarize our key contributions as follows:
\begin{enumerate}
    \item We 
    % operationalize distributional alignment \NB{personally don't love the operationalize buzzword---does this mean you define the objective of DA?}, and 
    identify three critical sources of variation in distributional alignment (the question, the steering method, and the output type) and construct a benchmark based on these dimensions.
    \item We collect a new dataset on distributional alignment, NYT Books, that expands measurements beyond political and cultural values. 
    \item We perform an analysis of our benchmark design choices, finding several open problems for the field: (1) Log-probability based metrics for distributional alignment may systematically underestimate LM performance (2) LMs may `know' about distributional alignment but are unable to sample from its own distribution (3) Persona steering simulates more polarized humans.
    % \NB{Can you possibly make 1 and 2 a single contribution that is also a suggestion of best practices, kind of like Katherine's "just ask for calibration" paper's pitch? Like "verbalized distributions tend to outperform sampling-based methods of extracting distributions"}


% While some have used distributional differences to measure how models are biased ~\citep{santurkar2023opinions, durmus2024measuring}
% %angelina’s paper, political compass, what citeps these, argyle - persona}, 
% there is still a limited understanding of how practitioners can best \textit{control} or \textit{steer} the distributions of model outputs under deployment. 



% In settings such as personalization, an important measure of performance is an LLM’s ability to adapt to represent the opinion of various demographic groups. 


% However, when researchers measure to which group of people a model best aligns or try to steer a model towards specific values, they often compare average responses which does not capture the diversity of responses a group may hold. Representing a group as the average of responses from that group removes all variation in responses, treating what should be additional information as noise. A recent line of work \citep{sorensen2024roadmap} has advocated for comparing distributions of responses as it leads to clearer results and better characterization of models.


% Several have pointed out flaws in such work, including stereotyping of demographic groups \citep{cheng2023marked}, and misportraying and flattening the representations of
% demographic groups \citep{wang2024large}. For these reasons, we
% caution against use cases where LLMs are intended to replace human participants, and point out that when using LLMs to simulate human behavior, it's important to do so in a way that captures diversity in thought, not just caricatures or stereotypes. It motivates the task of \textit{distributional alignment}, not just alignment on average, as high performance on this task allows us to capture heterogeneity, coverage, and diversity in responses. 
% alignment on average = current state
% wiht out a distribution, you end up with stereotypes/essentialism of their properties

% getting distirbtioal alignment right allows us to capture heterogenity and diversity in responess, nand measure how good LMs are at capturing heterogeneity 
% can models get good coverage of ppl they want to simulate, people of various gruops have diverse opnions, yet models have unidimensional represetnations of people
% given particular attributes about pepole, can they model heterogeneity after conditioning

% Current models have not been extensively studied in terms of their distributional alignment. While some have used distributional differences to measure how models are biased ~\citep{santurkar2023opinions, durmus2024measuring}
% %angelina’s paper, political compass, what citeps these, argyle - persona}, 
% there is still a limited understanding of how practitioners can best \textit{control} or \textit{steer} the distributions of model outputs under deployment. 

 


% Previously distributional alignment work has framed their work as a "probe to enable developers to better understand model behavior and for users to identify and flag representation failures, and not as a benchmark, that should be indiscriminately optimized". However, in this paper we argue that if __, these gaps should be closed especially since we're operating in a setting 



% SKELETON OF PAPER: 
% There is an important problem X
% Models are bad at X
% Here is a table that shows you that models are bad at X 



% Main message: there are something models can do surprisingly well (much more knowledge intensive), but this simulation and capturing diversity of different views that appear is really missing in their capabilities. 




%    \item We evaluate these models and steering methods on three datasets for their ability to be steered towards the distribution of opinions/preferences of six target demographic groups.
    % \item Introduce a new dataset to measure distributional alignment
    % \item Highlighting challenges of using model log probabilities to measure distributional alignment 
    % \item simulation to knowledge gap: model log probs are bad but the knowledge is there 
    % models generate samples that are calibrated (sorenson)=model  VS 
    % there exists models that ask for alignemtn interms of log probs, but it can be aligned in other forms of sampling/elcitiation mechanism 

    


    % here are 3 failure modes people should be studying 
%    \item formalziatino of task 
\end{enumerate}





==> Sections/problemsetting_old.tex <==
\label{sec:problemsetting}

\NB{why is the whole section "problem statement"? It feels like a lot of the section is just all the details of the benchmark, so maybe you should put the next section header earlier?}
\irena{+1, and actually a problem statement section would be great! You could use it to offer some definitions for distributional alignment. }

% We propose a benchmark that systematically evaluates the extent to which a language model
% We propose a benchmark that systematically evaluates the extent to which a language model can be aligned to the distribution of a particular demographic group's opinions. We begin with a definition of distributional alignment (Sec. \ref{sec:problemsetting-def}). Then, we explore the ways in which a model can be distributionally aligned (Sec. \ref{sec:problemsetting-ways}). Finally, we demonstrate that models have a simulation to knowledge gap, a key limitation if practitioners want to simulate the opinions of demographic groups (Sec. \ref{sec:problemsetting-gap}). 

% We propose a benchmark that systematically evaluates the extent to which a language model can be aligned to the distribution of a particular demographic group's opinions. We begin by defining relevant concepts (Sec. \ref{sec:problemsetting-def}, \ref{sec:problemsetting-alignment}). We then present a simple example of simulating a biased coin, which highlights the importance of carefully validating \emph{how} we measure distributional alignment (Sec. \ref{sec:problemsetting-toyprob}).


We propose a benchmark that systematically evaluates the extent to which a language model can be aligned to the distribution of a particular demographic group's opinions, a task we term the \textit{distributional alignment problem}.
\NB{I didn't realize that you were actually framing this problem until this point in the paper---I think the issue is that the word "operationalize" is very vague. Maybe literally just say you define distributional alignment, and then define it, early in the introduction?}
%Given a dataset that is providing a distribution over questions. we are asking if a LM can reproduce the quantity. We explore a lm M representing group g. we explore ways of doing this through steering methods S.this will generate \hat{y}_{g, q}. Our goal is to evaluate if y and y hat are close (no equatioN)
\NB{you should definitely have a concrete example in this paragraph. Just giving the notation is sort of confusing. e.g., come up with a question, a group, and an example of $y_{g, q}$ (favorite ice cream, people 18-30 years old)}
In this problem, we are given a dataset with distribution $y_{g,q}$ across multiple choices answers for each question $q$ and group $g$. The goal is to understand how a language model $M$ can represent a group $g$ through a steering method $S$, one that shifts an LM's opinion distribution to that of a particular group. Concretely, the model will estimate a distribution $\hat{y}_{g,q}$ and we evaluate the distributional difference between the reference distribution, $y_{g,q}$, and the model's estimate, $\hat{y}_{g,q}$ (Fig. \ref{fig:fig1}).
% \irena{Oh, okay! This immediately resolves most of my questions in the intro. Can you make this more clear in the intro, that you're in this multiple choice setting? This is very different from the impression I got early in the intro, which is that you were also interested in the full-on generative setting (evaluating full monologues of different personas)}
% \irena{Another thing I think is worth noting is that the definition of distributional alignment seems like it needs to change depending on what kind of data you have from the human population of interest. Multiple choice answers is one thing, but what if you only have written text from the humans? Then this definition is insufficient.}
% language model $M$, a steering method $S$ for group $g$, and a reference distribution $y_g$ of actual samples from people in group $g$. The alignment algorithm produces $M( q | S_g)$ that aims to imitate $y_g$. Finally, we evaluate the distributional difference between the model output and reference distribution, $D( M(\cdot | S_g, y_g)$.
% Instantiating each of these components involves a number of details, which we describe below. 

In this section, we formalize the steering method, output type, and evaluation metric.
% In this section, We walk through the three core components of the task: the input (Sec. \ref{sec:problemsetting-input}), output (Sec. \ref{sec:problemsetting-output}), and evaluation metric (Sec. \ref{sec:problemsetting-eval}).  



% We then describe how prior work uses model log-probabilities to measure the distributional output (Sec. \ref{sec:problemsetting-prior}). We highlight the shortcomings of this distribution estimation methods and propose alternatives (Sec. \ref{sec:problemsetting-alt}). 

% present a simple example of simulating a biased coin, which highlights the importance of carefully validating \emph{how} we measure distributional alignment (Sec. \ref{sec:problemsetting-toyprob}).



% Sec 2.1: Definitions, Set up knowledge vs sampling
% Define what it means for a model to know something: a model knows something when given a prompt the outputs can be mapped to the distribution (verbalize distribution)
% Define Sampling: some procedure that can be viewed as a sampler (not iid) (either prompting or log probs) something that generates a sample - we can measure the marginal distribution of the sample
% Introduce total variation
% Question: Do we want to keep this paragraph/notation? I agree that it doesnt really define notation for later, but is there a way it can be edited so that it does?

% The high-level goal is to quantify how much a language model can be steered towards the distribution of opinions of a particular target demographic group. 





% \subsection{Definitions} \label{sec:problemsetting-def}

% The goal of distributional alignment is to evaluate the extent to which a model is steered towards a distribution over answers compared to a given population. In this section, we introduce each component of the task, as depicted in Fig. \ref{fig:fig1}, building upon notation set forth in \citet{sorensen2024roadmap} and \citet{santurkar2023opinions}.

% % pre-req: dataset 
% First, we need a dataset of group opinion distributions against which we can compare to LMs. We can build this by aggregating human survey responses and stratifying based on demographic group. Let $Q$ be set of survey questions to which humans in group $G$ have a distribution $Y$ over the set of possible multiple-choice answers.

% % input: steering method
% Next, as input to our model $M$, we need a steering method $S$ to align $M$ to $G$ (Sec. \ref{sec:problemsetting-input}). 
% % output distribution estimation methods
% Then, to obtain the output distribution of model opinions across survey questions, $\hat{Y}$, we prompt the model for the group's distribution across answer choices. This can be measured in several ways, and in Sec. \ref{sec:problemsetting-output} we show there is sensitivity to the distributional output type. 

% Finally, to quantify the amount $S$ steers $M$ towards the opinions of $G$, we use a distributional comparison metric that captures the similarity between the ground truth group distribution $Y$ and model estimate of the group distribution $\hat{Y}$ (Sec. \ref{sec:problemsetting-eval}).  


\subsection{Input: Steering Method}
\label{sec:problemsetting-input}

%Goal: there are a couple different steering methods, steering methods are important. 
Steerability in the context of this work refers to a LM’s ability to adapt to represent the opinion of a target demographic group.
We evaluate two steering methods, persona and few-shot steering, by prepending additional context to the prompt describing the group we want the model to emulate. 
We study these variations as existing techniques such as persona steering are known to be inaccurate, and these errors lead to undesirable side effects including stereotyping, exacerbating polarization, and creating echo chambers \citep{perez2022discovering, cheng2023marked, wang2024large}.

% Persona Steering
\textbf{Persona Steering}: 
\citet{cheng2023marked} define a persona as a ``natural language portrayal of an imagined individual belonging to some (intersectional) demographic group.'' In persona steering, we append such a persona as part of a prompt, asking the language model to emulate behavior from this group. Concretely, we follow a version of persona steering from \citet{santurkar2023opinions,Kambhatla} where the LM is instructed to pretend to be a member of target demographic group (e.g. ``Please simulate an answer from a group of Republicans.").

% Few Shot
\textbf{Few Shot Steering}: 
Despite the popularity of persona steering, prior work has found several limitations to persona steering such as stereotyping and social bias \citep{santurkar2023opinions,liu2024evaluating,wang2024large}.
Inspired by the success of few-shot prompting in language understanding tasks \citep{NEURIPS2020_1457c0d6}, 
we construct a few shot setting in which in-context examples of ground truth  group opinion distributions are provided in the prompt. More specifically, LMs are given five examples of similar questions and their corresponding ground truth distribution from a group. Then, they are instructed to simulate an answer from that group. This few shot setting is representative of real-world distributional alignment tasks as practitioners often have access to existing surveys and ground truth opinion distributions on similar questions. 
% of a few shot steering method in which in-context examples of ground truth group opinion distributions are provided in the prompt. 

% From prior work that finds limited success for persona steered distributional alignment \citep{santurkar2023opinions,liu2024evaluating}, we also implement a few shot steering method in which in-context examples of ground truth group opinion distributions are provided in the prompt. 

% \citet{santurkar2023opinions,liu2024evaluating} study persona steered models and find limited success for distributional alignment, suggesting that alternative methods are needed.
% It has been observed that integrating task demonstrations is highly useful for language understanding tasks \citep{NEURIPS2020_1457c0d6}, motivating the study of a few shot steering method in which in-context examples of ground truth group opinion distributions are provided in the prompt. 

% \nicole{todo: it's hard to go from a persona, we make the task easier with few shot stuff; Success with in-context learning in LMs motivates us to study different types of settings like few shots where there might be more possibilities in actually being aligned; incontext few shot gpt stuff, in other NLP/language understanding tasks it has been observed that giving examples of the task is highly useful. Inspired by these success, we evaluate a few shot setting in which we give examples of surveys. Here is one such example of a few shot prompt.}

% Comparison 
% A comparison across two steering methods elucidates information that is most relevant to align model responses to the opinions of a human group and reveals scenarios in which one steering method may be more suitable than others. 



% For example, persona steering has been shown to have undesirable side-effects including stereotyping, exacerbating polarization, and creating echo chambers \citep{perez2022discovering, cheng2023marked, wang2024large}. 
% While persona steering is well-studied \citep{liu2024evaluating,wang2024large,cheng2023marked,santurkar2023opinions}, it is unclear how persona steering compares to models steered with ground truth group opinion distributions on similar questions. 

% \nicole{todo: justify few shot and cite prior work that suggests it might be a good idea, difference between the two; }

\subsection{Output: Distributional Output Type}
\label{sec:problemsetting-output}

% Describe how the output needs to represent a distribution and how one might do that : Our surveys are MC and we can ask LMs to answer them; we need a distribution, how should we get this distribution? 

When LMs are asked to emulate a population's response to a multiple-choice survey question, there is no single ``correct" answer choice. Instead, the model output should match the \textit{distribution} of model opinions for each question across the set of multiple-choice answers. 
% \NB{I feel like this point is v important and should be conveyed in the introduction, when you define distributional alignment}


% In our benchmark we are going to consider 3 ways of distribution estimation:  Present the 3 ways
To obtain this distribution, we prompt the model and extract an opinion distribution in three ways: measuring model log-probabilities, prompting an LM for a sequence of answer choices, and directly verbalizing distributional knowledge. In this section, we describe these three distributional output types \NB{see note in figure 1 about switching from output types to "modes of expressing opinion distributions"} and demonstrate that the distributional alignment accuracy is highly sensitive to the distribution estimation method. \NB{and maybe switching distribution estimation to distribution expression?}

% Previous work used log-probs, but there are issues. 
\textbf{1. Model Log-probabilities: }A natural distribution estimation method is to measure the model's log-probabilities of the next token response for each answer choice \citep{santurkar2023opinions, durmus2024measuring}; however, prior work has highlighted limitations of using this technique, specifically that model log-probabilities struggle to replicate a ground truth distribution. For example, \citet{durmus2024measuring} find that model log-probabilities have a concentrated probability mass on a few answer choices, especially in models trained with Reinforcement Learning from Human
Feedback (RLHF) \citep{christiano2023deepreinforcementlearninghuman}, rather than more dispersed answers as seen in their corresponding human distributions.

\textbf{2. Sequence of Tokens: }While model log-probabilities represent the result of drawing samples from a LM,
% \NB{are you saying here that you estimate log probs with sampling? this is new to the reader I think, so maybe should state this more clearly---this is also just because you're operating in the API setting right? that should be explained somewhere}, 
a model can also express its distributions by behaving as a sampler and emit a sequence of samples from the distribution (e.g., \texttt{ABBBAABDDBACBDB}). This may be advantageous when practitioners 
want to generate samples from an opinion distribution for simulation purposes.
% exclusively use a language model for both sampling and distribution estimation (i.e., no external sampler). 
%This represents a model's ability to simulate its knowledge of a distribution.

\textbf{3. Verbalize Distributional Knowledge: } 
% \NB{I think you should try to stick to a specific terminology for each of these expression methods. A good way to stay consistent is to write out a table with all your notation and terms of art, and make sure you stick with it when writing the paper} 
Lastly, we can remove the requirement that models must sample from simulated humans and instruct a model to directly verbalize the distribution in the output text, without an estimation procedure or post-processing applied (e.g., text in a JSON format \texttt{\{A: 25\%, B: 20\%, C: 45\%, D: 10\%\}}).\footnote{While this verbalized knowledge can be fed into an external random sampler, it is not a sufficient output for downstream applications (e.g., in the case of piloting surveys) and existing approaches to simulating humans do not take this approach (cite simulacra paper, other recent papers on generating personas). Our later results suggest this approach may be fruitful as a distributional alignment method.}
% as practitioners often exclusively use a language model for both sampling and distribution estimation \citep{todo}.
This differs from the aforementioned distributional output types in that this separates distributional knowledge from the LM's ability to also generate samples. 





\begin{figure*}[ht!]
  \centering
  \includegraphics[width=\textwidth]{Figures/biasedcoinflip (7).pdf}
  \caption{\textbf{Biased Coin Flip Experiment}: We find that when the probability of heads is measured via model log-probabilities as shown in blue, the results are highly uncalibrated. This behavior is mitigated with temperature scaling (TS), shown in green. However, when the distribution is expressed through emitting a 30-flip sequence of H-T (Sequence) or directly verbalizing the distributional knowledge (Verbalize Knowledge), we do not observe the same mis-calibration issue.}
\label{fig:biasedcoin}
\end{figure*}

% Simple experiment to show this log prob weakness. 
\textbf{These three estimation methods reveal surprising performance gaps.} Consider a toy experiment in which the model has \textit{full knowledge} of the ground truth distribution.
% Due to the __ of model log-probabilities, verbalize and sequence turn out to the extracted distribution is highly sensitive to the distribution estimation method.
% We demonstrate the magnitude of this issue with a toy experiment in which the model has \textit{full knowledge} of the ground truth distribution.
In this experiment, an LLM is instructed to simulate a flip of a biased coin which has $P(H)=p$ and $P(T)=1-p$. Naturally, we would expect the model log-probabilities for the token `H' to be $p$ and `T' to be $1-p$. In reality, we see that the model log-probabilities are highly un-calibrated. They provide a misleading picture of the ground truth distribution, despite the fact that the ground truth distribution is shared in the input prompt (Fig. \ref{fig:biasedcoin}). Moreover, we find that two other distributional estimation methods do not suffer the same mis-calibration issue: both verbalizing the distribution and emitting a sequence of 30 samples of the biased coin flip are much more calibrated than the model's log-probabilities.\footnote{This type of performance gap is not unexpected; it has been shown that while models excel in text and image generation tasks (knowledge), they fall short when asked to validate if the generated answer is correct \citep{li2023benchmarking,west2023generative}.}
% \NB{the samples aren't IID though right? (otherwise they should do exactly as well as the log probs?) maybe should mention this, idk}




% This problem is fixed by using the other estimations → show sensitivity to distribution method  : Set up / motivate knowledge to simulation gap . We term this knowledge to simulation gap

% \nicole{todo: commentary on knowledge to sim}


Results from this biased coin flip experiment suggests two things: (1) prior distributional alignment work using model log-probabilities may not be seeing the full picture and (2) there exists a significant performance gap, one that we term \textit{knowledge-to-simulation gap}. This gap refers to instances where models may have alignment in knowledge (i.e., verbalizing the distribution in the output text), but not in sampling behavior (i.e., as measured via model log-probabilities or emitting a sequence of tokens). 

% Broadly speaking, a model \textit{knows} a distribution when given a prompt, the output is directly mapped to a group distribution, without an estimation procedure or post-processing applied to the output. This can take form of verbalizing the distribution in the output text (e.g., in a json format \texttt{\{A: 25\%, B: 20\%, C: 45\%, D: 10\%\}}).

% A model is aligned in its \textit{sampling behavior }when it emits a distribution with some procedure that can be viewed as a sampler (not necessarily i.i.d) either through sampling from the model with model log-probabilities or prompting the model to simulate $n$ samples of a target group and emit a sequence of answer choices (e.g., \texttt{‘AABBAABBCC’}). We can compute the marginal distribution of output sample over the set of possible answer choice selection. 

% When using model log-probabilities, we are viewing the model as a \textit{sampler}, sampling from the model's distribution over each answer choice. However, we can also view the model as a \textit{generator}, generating the knowledge distribution directly by verbalizing the distribution in its outputs. 

% \nicole{some sort of transition}

% This difference in performance when viewing the model as a sampler or generated exemplifies limitations that our benchmark captures. and we intentionally characterize these 

% \subsection{Implications}
% \label{sec:problemsetting-implications}

% Describe how distribtional alignment is measured currently: model log probs






\subsection{Evaluation: Measuring Distributional Alignment}
\label{sec:problemsetting-eval}
Given that we have defined a procedure by which we can extract opinion distributions conditioned on demographic groups, what remains to complete the benchmark is an evaluation metric for how close the model's opinion distribution is to ground truth opinion distributions. Our benchmark ranks models based on the total variation distance between the model's distribution estimate and the human opinion distribution.

% More formally, we define the distributional alignment of a model instructed to express its distribution with output type $O$ as 

% $$\mathcal{A}(Y,\hat{Y}_{S, \mathcal{O}}) = \frac{1}{|G|} \sum_{g \in G}  \frac{1}{|Q|} \sum_{q \in Q} \frac{1}{2} {\left \lvert\lvert y_{g, q}- \hat{y}_{g, q} \right \rvert\rvert}_1 ,$$
% \NB{I would define all of the below notation before you write the equation. "Let x be the ABC"}

% where $G$ is the set of demographic groups, $q \in Q$ is a survey question to which respondents from group $g$ have an opinion distribution $y_{g,q}$.\footnote{Note that for each question $q$, there can be a different number of answer choices. Thus, the dimensionality of $y_{g,q}$ depends on $q$.} We apply a steering method $S$ to align the model towards $g$ and produce a distribution estimate, $\hat{y}_{g, q}$. Then, we can define our dataset as 
% $Y = \{ y_{g,q} \mid 1 \leq g \leq G, 1 \leq q \leq Q \}$, and our predicted distributions as 
% $\hat{Y}_{S, \mathcal{O}} = \{ \hat{y}_{g, q} \mid 1 \leq g \leq G, 1 \leq q \leq Q \}$.






Let $G$ be the set of demographic groups and $q \in Q$ be a survey question to which respondents from group $g$ have an opinion distribution $y_{g,q}$.\footnote{Note that for each question $q$, there can be a different number of answer choices. Thus, the dimensionality of $y_{g,q}$ depends on $q$.} We apply a steering method $S$ to align the model towards $g$ and produce a distribution estimate, $\hat{y}_{g, q}$. Then, we can define our dataset as 
$Y = \{ y_{g,q} \mid 1 \leq g \leq G, 1 \leq q \leq Q \}$, and our predicted distributions as 
$\hat{Y}_{S, \mathcal{O}} = \{ \hat{y}_{g, q} \mid 1 \leq g \leq G, 1 \leq q \leq Q \}$. The \textbf{distributional alignment} of a model instructed to express its distribution with output type $O$ as 
$$\mathcal{A}(Y,\hat{Y}_{S, \mathcal{O}}) = \frac{1}{|G|} \sum_{g \in G}  \frac{1}{|Q|} \sum_{q \in Q} \frac{1}{2} {\left \lvert\lvert y_{g, q}- \hat{y}_{g, q} \right \rvert\rvert}_1 .$$
We compute the metric as the average total variation between these two distributions which is bounded between 0 and 1, with a smaller number representing a higher 
performance on the task. 

% \NB{It feels slightly weird to define this knowledge-to-simulation thing here since this depends on the results -- can you just put it in your results section?}
The \textbf{knowledge-to-simulation gap} is the difference between the performance between verbalizing the distribution and emitting a sequence of answer choices.\footnote{The gap can also defined as the difference in performance between verbalize and model log-probabilities, yet our later results show model log-probabilities to not be competitive.} More formally, this gap is: 
$$\text{KS}_S = \mathcal{A}(Y,\hat{Y}_{S, {\text{Verbalize}}}) - \mathcal{A}(Y,\hat{Y}_{S, {\text{Sequence}}}) .$$
% \nicole{note: sequence always performs better than log probs}





==> Sections/relatedwork_old.tex <==
\label{sec:relatedwork}
% \nicole{work in progress. \href{https://docs.google.com/document/d/1n2du63IVSFQGgSQpSRqgutZuPNo8LK15bivDPEPDFi8/edit}{Link to outline and consolidation of related works}}


% \NB{this is an impressively long related work, I feel like you may need to shorten lol}

\textbf{Distributionally Pluralistic Alignment. }
LLMs often learn an averaged human preference and struggle to model diverse preferences across groups, leading to a growing body of work advocating for \textit{distributionally pluralistic models} \citep{sorensen2024roadmap,feng2024modularpluralismpluralisticalignment,kirk2024prismalignmentprojectparticipatory, chen2024palpluralisticalignmentframework} that are well-calibrated to the distribution of responses to a given population. However, \citet{sorensen2024roadmap} acknowledge there is limited knowledge of explicit alignment procedures to explicitly increase distributional calibration, highlighting the 
importance of our work in characterizing key sources of variation and how they affect quantitative measurements of distributional alignment.



\textbf{LLMs to simulate human behavior.}
With the proliferation of LLMs, there is an emerging body of research that integrates LLMs into computational social science to perform tasks such as simulating social psychology experiments \citep{pmlr-v202-aher23a,DILLION2023597} or human-like agents \citep{park2023generative,samuel2024personagymevaluatingpersonaagents,horton2023largelanguagemodelssimulated}
% \citep{park2023generative,samuel2024personagymevaluatingpersonaagents,horton2023largelanguagemodelssimulated,chuang2024simulatingopiniondynamicsnetworks,wang2023humanoidagentsplatformsimulating}
, and annotating data \citep{he2024annollmmakinglargelanguage,doi:10.1177/20531680241231468} to name a few. We focus on a popular use case -- LLMs simulating humans to generate survey samples \citep{hwang2023aligning, zhou2024sotopia, pmlr-v202-aher23a, ziems2024large, Argyle_2023,
10.1145/3544548.3580688} and predict opinions \citep{kim2024aiaugmentedsurveysleveraginglarge,jiang2022communitylmprobingpartisanworldviews}. 

Despite this surge of excitement, several works urge caution when relying on the survey responses of LLMs to elicit synthetic responses, citing concerns such as group stereotyping and misrepresentation \citep{wang2024large,abdurahman_perils,geng2024largelanguagemodelschameleons}, preference for socially desirable responses \citep{ai2024cognitionactionconsistentnot}, 
lower entropy in model responses \citep{dominguezolmedo2024questioningsurveyresponseslarge,park2023diminisheddiversityofthoughtstandardlarge}, and answer inconsistencies from prompt brittleness \citep{ceron2024promptbrittlenessevaluatingreliability}.
% lower entropy in model responses \citep{dominguezolmedo2024questioningsurveyresponseslarge,durmus2024measuring,abdurahman_perils,Bisbee_Clinton_Dorff_Kenkel_Larson_2024,park2023diminisheddiversityofthoughtstandardlarge,ziems2024large}, and answer inconsistencies from prompt brittleness \citep{dominguezolmedo2024questioningsurveyresponseslarge,ceron2024promptbrittlenessevaluatingreliability,Bisbee_Clinton_Dorff_Kenkel_Larson_2024,röttger2024politicalcompassspinningarrow,lyu2024probabilitiesunveilingmisalignmentevaluating,wang2024myanswercfirsttoken}.
% , and answer inconsistencies (e.g., prompt brittleness \citep{Bisbee_Clinton_Dorff_Kenkel_Larson_2024}, differences when convert multiple-choice surveys to free text \citep{röttger2024politicalcompassspinningarrow,lyu2024probabilitiesunveilingmisalignmentevaluating,wang2024myanswercfirsttoken}, answer choice order bias \citep{dominguezolmedo2024questioningsurveyresponseslarge}, and limited robustness to negation or inversion \citep{ceron2024promptbrittlenessevaluatingreliability}). 
While these works provide important context for understanding the limitations of LLMs in emulating human behavior, they focus on zero-shot and political or cultural values leaving several sources of variation unexamined. The closest work to ours is \citet{dominguezolmedo2024questioningsurveyresponseslarge} who study answer choice order bias and find that model responses have different variation than that of humans. Our work is distinct in that we don't focus on stability with respect to prompt variation. Instead, we look at higher level design choices such as the steering method (e.g. few shot) and distribution estimation method that significantly affect alignment measurements. 

% we improve our understanding of three different variables: the dataset, steering method, and distributional output type. \nicole{how to make this stronger?}. 

Next, we describe existing research on these variables and how our work makes new contributions.

\textbf{Dataset.}
\citet{santurkar2023opinions} evaluate how model responses to Pew American Trends Panel survey questions align with survey respondents from different
demographics, inspiring numerous works that adopt this methodology to quantify alignment through responses to cultural surveys \citep{durmus2024measuring,naous2024havingbeerprayermeasuring,wang2024countriescelebratethanksgivingcultural,pistilli2024civicsbuildingdatasetexamining,kovač2023largelanguagemodelssuperpositions,masoud2024culturalalignmentlargelanguage,zhao2024worldvaluesbenchlargescalebenchmarkdataset,Sorensen_2024} and political surveys \citep{stammbach2024aligninglargelanguagemodels,röttger2024politicalcompassspinningarrow}. 
However, there is limited knowledge of how models respond to non-political yet subjective values, such as product preferences.\footnote{\citet{namikoshi2024usingllmsmodelbeliefs} align models to the preferences of real human respondents on a survey of preferences for battery electric vehicles, yet this dataset is not available to download.} This gap motivates our contribution of the NYT Books dataset.

\textbf{Steering Method.}
The literature has studied a variety of methods to steer the generation of LLMs toward specific opinions. A popular method of steering is persona steering, where LMs are steered based on demographic group traits. This can be achieved by prepending demographic information (such as Democratic or Republican affiliations) to prompts \citep{santurkar2023opinions,simmons2023moralmimicrylargelanguage,perez2022discovering,cheng2023marked,liu2024evaluating,samuel2024personagymevaluatingpersonaagents,giorgi2024explicitimplicitlargelanguage,castricato2024personareproducibletestbedpluralistic,hu2024quantifyingpersonaeffectllm}, prepending past opinions \citep{hwang2023aligning}, and fine-tuning \citep{jiang2022communitylmprobingpartisanworldviews,namikoshi2024usingllmsmodelbeliefs}. 
It is important to note that recent research has raised concerns that persona-steered generation leads to more toxic outputs \citep{gupta2024biasrunsdeepimplicit,salewski2023incontextimpersonationrevealslarge,wang2024large,cheng2023marked,cheng2023compostcharacterizingevaluatingcaricature,wan2023personalizedstochasticparrotsdangerous,deshpande2023toxicitychatgptanalyzingpersonaassigned}, motivating our disaggregated analysis \citep{barocas2021designingdisaggregatedevaluationsai}. In addition to persona steering, prior works have also focused on steering with in-context examples \citep{kim2024fewshotpersonalizationllmsmisaligned,zhao2023grouppreferenceoptimizationfewshot}, prefix-tuning with persona grounded in collaborative filtering \citep{li2024steerabilitylargelanguagemodels}, modifying activations in the forward pass \citep{turner2024activationadditionsteeringlanguage}, and creating human belief networks \citep{chuang2024demographicsaligningroleplayingllmbased}. 
Closest to our work is 
\citet{santurkar2023opinions} and \citet{liu2024evaluating} who evaluate persona steering in their analysis, yet in our steerability analysis we consider cases in which practitioners have access to prior survey data and can use it as few shot examples. 

\textbf{Distribution Expression Method.} Prior work has found inconsistencies in the model's expressed opinions. For example, \citet{Bisbee_Clinton_Dorff_Kenkel_Larson_2024} find that the distribution of synthetic responses sensitive to minor changes in prompt wording, and \citet{ceron2024promptbrittlenessevaluatingreliability} find similar results when negating or inverting survey question. Furthermore, there are also inconsistencies when converting multiple-choice surveys to free text \citep{röttger2024politicalcompassspinningarrow,lyu2024probabilitiesunveilingmisalignmentevaluating,wang2024myanswercfirsttoken}, and shuffling the order of the survey answer choices \citep{dominguezolmedo2024questioningsurveyresponseslarge}. 
When evaluating LLMs on the basis of survey questions, \citet{santurkar2023opinions}, and all the works that have followed, study models’ probability distribution over various answer choices. Recent work has begun to explore how to better sample from LMs \citep{zhu2024recoveringmentalrepresentationslarge,requeima2024llmprocessesnumericalpredictive} and use LMs for probabilistic reasoning \citep{paruchuri2024oddslanguagemodelscapable}, but do not apply it to the simulating opinion distributions. 
We explore differences in distribution expression and take inspiration from work that suggests verbalized uncertainty can be competitive with model log-probabilities \citep{tian2023justaskcalibrationstrategies}.

